Probabilistic proofs of large deviation results for sums of semiexponential random variables and explicit rate function at the transition

Asymptotics deviation probabilities of the sum S n = X 1 + $\times$ $\times$ $\times$ + X n of independent and identically distributed real-valued random variables have been extensively investigated, in particular when X 1 is not exponentially integrable. For instance, A.V. Nagaev formulated exact asymptotics results for P(S n > x n) when x n > n 1/2 (see, [13, 14]). In this paper, we derive rough asymptotics results (at logarithmic scale) with shorter proofs relying on classical tools of large deviation theory and expliciting the rate function at the transition.

==> commath.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Commandes mathématiques
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\RequirePackage{babel}					%Pour les commandes dépendant de la langue du document
\RequirePackage{amsmath}				%Math de l'AMS
\RequirePackage{amssymb}				%Autres symboles mathématiques
\RequirePackage{amsthm}					%Théorèmes correctement organi}és
\RequirePackage{bbm}					%Fonction indicatrice
\RequirePackage{stmaryrd}				%Crochets pour les intervalles entiers

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Rémi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% Making \big, etc. a relative size rather than absolute (with default parameters, ex is 4.3045 pt)
%
%\renewcommand\big[1]{{\hbox{$\left#1\vbox to 1.97ex{}\right.\n@space$}}}
%\renewcommand\Big[1]{{\hbox{$\left#1\vbox to 2.67ex{}\right.\n@space$}}}
%\renewcommand\bigg[1]{{\hbox{$\left#1\vbox to 3.37ex{}\right.\n@space$}}}
%\renewcommand\Bigg[1]{{\hbox{$\left#1\vbox to 4.07ex{}\right.\n@space$}}}
%
%% Paired delimiters
%
%\DeclarePairedDelimiter\abs\lvert\rvert % Absolute value
%\DeclarePairedDelimiter\brack\lbrack\rbrack % Brackets
%\DeclarePairedDelimiter\ceil\lceil\rceil % Ceiling
%\DeclarePairedDelimiter\floor\lfloor\rfloor % Floor
%\DeclarePairedDelimiter\intervalicc\llbracket\rrbracket % Closed integer interval
%\DeclarePairedDelimiter\intervalico\llbracket\llbracket % Closed-open integer interval
%\DeclarePairedDelimiter\intervalioc\rrbracket\rrbracket % Open-closed integer interval
%\DeclarePairedDelimiter\intervalioo\rrbracket\llbracket % Open interger interval
%\DeclarePairedDelimiter\norm\lVert\rVert % Norm
%\DeclarePairedDelimiter\paren() % Parentheses
%\DeclarePairedDelimiter\set\{\} % Set
%
%\DeclarePairedDelimiterX\inner[2]\langle\rangle{#1,#2} % Inner product
%\DeclarePairedDelimiterX\intervalcc[2]\lbrack\rbrack{#1,#2} % Closed interval
%\DeclarePairedDelimiterX\intervalco[2]\lbrack\rparen{#1,#2} % Closed-open interval
%\DeclarePairedDelimiterX\intervaloc[2]\lparen\rbrack{#1,#2} % Open-closed interval
%\DeclarePairedDelimiterX\intervaloo[2]\lparen\rparen{#1,#2} % Open interval
%\DeclarePairedDelimiterX\setst[2]\{\}{#1\ \delimsize|\ #2} % Set of the #1 such that #2
%
%% Use of some characters from the Fourier-GUTenberg package
%
%\DeclareFontEncoding{FMS}{}{}
%\DeclareFontSubstitution{FMS}{futm}{m}{n}
%\DeclareFontEncoding{FMX}{}{}
%\DeclareFontSubstitution{FMX}{futm}{m}{n}
%\DeclareSymbolFont{fouriersymbols}{FMS}{futm}{m}{n}
%\DeclareSymbolFont{fourierlargesymbols}{FMX}{futm}{m}{n}
%\DeclareMathDelimiter{\llbracket}{\mathopen}{fouriersymbols}{153}{fourierlargesymbols}{133}
%\DeclareMathDelimiter{\rrbracket}{\mathclose}{fouriersymbols}{154}{fourierlargesymbols}{134}
%\DeclareMathDelimiter{\VERT}{\mathord}{fouriersymbols}{152}{fourierlargesymbols}{147}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Mathématiques générales
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%Ensembles de nombres
\newcommand{\ensnombre}[1]{\mathbb{#1}}%
\newcommand{\N}{\ensnombre{N}}
\newcommand{\Z}{\ensnombre{Z}}
\newcommand{\Q}{\ensnombre{Q}}
\newcommand{\R}{\ensnombre{R}}
\newcommand{\C}{\ensnombre{C}}

%Divers
\newcommand{\card}[1]{\left\lvert #1 \right\rvert}

\DeclareMathOperator{\id}{id}

\renewcommand{\Re}{\mathfrak{Re}}
\renewcommand{\Im}{\mathfrak{Im}}

\newcommand{\abs}[1]{\left\lvert #1 \right\rvert}
\newcommand{\norme}[1]{\left\lVert #1 \right\rVert}
\newcommand{\prodscal}[2]{\left\langle {#1} \mathrel{}\middle|\mathrel{} {#2} \right\rangle}
\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}
\newcommand{\ceil}[1]{\left\lceil #1 \right\rceil}

\newcommand{\ensfonction}[3]{#1(#2 ; #3)}
\newcommand{\enstq}[2]{\left\{ #1 \mathrel{}\middle|\mathrel{} #2 \right\}}
\newcommand{\ensavec}[2]{\left\{ #1 \mathrel{};\mathrel{} #2 \right\}}
\newcommand{\enspart}{\mathfrak{P}}

\newcommand{\defeq}{\mathrel{\mathop:}=}
\newcommand{\eqdef}{\mathrel{=}:}

\newcommand{\seq}[1]{#1}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Algèbre linéaire
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\ensmatrice}[3]{\mathcal{#1}_{#2}(#3)}

\newcommand{\transposee}[1]{{#1}^\top}
%\newcommand{\transposee}[1]{{}^t\! #1}

\DeclareMathOperator{\Vect}{Vect}
\DeclareMathOperator{\rg}{rg}
\DeclareMathOperator{\Ima}{Im}
\DeclareMathOperator{\Ker}{Ker}
\DeclareMathOperator{\tr}{tr}
\DeclareMathOperator{\Com}{Com}
\DeclareMathOperator{\Mat}{Mat}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Probabilités
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\indic}{\mathbbm{1}}
\newcommand{\Prob}{\mathbb{P}}
\newcommand{\Loi}{\mathcal{L}}
\newcommand{\Espe}{\mathbb{E}}
\newcommand{\ET}{\sigma}
\DeclareMathOperator{\Var}{Var}
\DeclareMathOperator{\Cov}{Cov}
\newcommand{\complementaire}[1]{{}^c\! #1}

\newcommand{\Probcond}[2]{\Prob\left( #1 \mathrel{}\middle|\mathrel{} #2 \right)}
\newcommand{\Loicond}[2]{\Loi\left(#1 \mathrel{}\middle|\mathrel{} #2 \right)}
\newcommand{\Especond}[2]{\Espe\left[ #1 \mathrel{}\middle|\mathrel{} #2 \right]}
\newcommand{\Varcond}[2]{\Var\left(#1 \mathrel{}\middle|\mathrel{} #2 \right)}




\iflanguage{french}%
{
%VERSION FRANCAISE

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Fonctions
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\let\cosh\relax
\DeclareMathOperator{\cosh}{ch}
\let\sinh\relax
\DeclareMathOperator{\sinh}{sh}
\let\tanh\relax
\DeclareMathOperator{\tanh}{th}

\DeclareMathOperator{\cotan}{cotan}
\DeclareMathOperator{\sinc}{sinc}
\DeclareMathOperator{\arcosh}{argch}
\DeclareMathOperator{\arsinh}{argsh}
\DeclareMathOperator{\artanh}{argth}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Intervalles
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\intervalle}[4]{\left#1#2\mathclose{}\mathpunct{},#3\right#4}%
\newcommand{\intervalleff}[2]{\intervalle{[}{#1}{#2}{]}}%
\newcommand{\intervalleof}[2]{\intervalle{]}{#1}{#2}{]}}%
\newcommand{\intervallefo}[2]{\intervalle{[}{#1}{#2}{[}}%
\newcommand{\intervalleoo}[2]{\intervalle{]}{#1}{#2}{[}}%
\newcommand{\intervallentff}[2]{\intervalle{\llbracket}{#1}{#2}{\rrbracket}}%
\newcommand{\intervallentof}[2]{\intervalle{\rrbracket}{#1}{#2}{\rrbracket}}%
\newcommand{\intervallentfo}[2]{\intervalle{\llbracket}{#1}{#2}{\llbracket}}%
\newcommand{\intervallentoo}[2]{\intervalle{\rrbracket}{#1}{#2}{\llbracket}}%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Théorèmes
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\theoremstyle{plain}%
\newtheorem{theorem}{Théorème}%
\newtheorem{lemma}{Lemme}%
%\newtheorem{lemma}[theorem]{Lemme}%
%\newtheorem{lemma}[section]{Lemme}%
\newtheorem{corollary}{Corollaire}%
\newtheorem{proposition}{Proposition}%
\newtheorem{property}{Propriété}%
\newtheorem{properties}{Propriétés}%
%
\theoremstyle{definition}%
\newtheorem{definition}{Définition}%
\newtheorem{hypothesis}{Hypothèse}%
\newtheorem{example}{Exemple}%
\newtheorem{examples}{Exemples}%
%
\theoremstyle{remark}%
\newtheorem*{remark}{Remarque}%
\newtheorem*{plus}{Complément}%
\theoremstyle{plain}%
}
{
%VERSION ANGLAISE

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Fonctions
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\DeclareMathOperator{\cotan}{cotan}
\DeclareMathOperator{\arcosh}{arcosh}
\DeclareMathOperator{\arsinh}{arsinh}
\DeclareMathOperator{\artanh}{artanh}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Intervalles
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\intervalle}[4]{\left#1#2,#3\right#4}%
\newcommand{\intervalleff}[2]{\intervalle{[}{#1}{#2}{]}}%
\newcommand{\intervalleof}[2]{\intervalle{(}{#1}{#2}{]}}%
\newcommand{\intervallefo}[2]{\intervalle{[}{#1}{#2}{)}}%
\newcommand{\intervalleoo}[2]{\intervalle{(}{#1}{#2}{)}}%
\newcommand{\intervallentff}[2]{\intervalle{\llbracket}{#1}{#2}{\rrbracket}}%
\newcommand{\intervallentof}[2]{\intervalle{\rrbracket}{#1}{#2}{\rrbracket}}%
\newcommand{\intervallentfo}[2]{\intervalle{\llbracket}{#1}{#2}{\llbracket}}%
\newcommand{\intervallentoo}[2]{\intervalle{\rrbracket}{#1}{#2}{\llbracket}}%

%\newcounter{intervallent}%
%\newcommand{\intervallentff}[2]{%
%	\setcounter{intervallent}{#1}%
%	\stepcounter{intervallent}%
%	\left\{#1,\theintervallent,\dots,#2\right\}}%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Théorèmes
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\theoremstyle{plain}%
\newtheorem{theorem}{Theorem}%
%
%\theoremstyle{definition}%
\newtheorem{lemma}[theorem]{Lemma}%
%\newtheorem{lemma}[theorem]{Lemma}%
%\newtheorem{lemma}[section]{Lemma}%
\newtheorem{corollary}[theorem]{Corollary}%
\newtheorem{proposition}[theorem]{Proposition}%
\newtheorem{definition}[theorem]{Definition}%
\newtheorem{property}[theorem]{Property}%
\newtheorem{properties}[theorem]{Properties}%
\newtheorem{hypothesis}[theorem]{Assumption}%
%\newtheorem{example}[theorem]{Exemple}%
\newtheorem{examples}[theorem]{Exemples}%
%
\theoremstyle{remark}%
\newtheorem*{remark}{Remark}%
\newtheorem*{plus}{Plus}%
}
